Mitigating Trauma in Qualitative Research Infrastructure: Roles for Machine Assistance and Trauma-Informed Design

Researchers increasingly look to understand experiences of pain, harm, and marginalization via qualitative analysis. Such work is needed to understand and address social ills, but poses risks to researchers' well-being: sifting through volumes of data on painful human experiences risks incurring traumatic exposure in the researcher. In this paper, we explore how the principles of trauma-informed computing (TIC) can be applied to reimagine healthier tools and workflows for qualitative analysis. We apply TIC to create a design provocation called TIQA, a system for qualitative coding that leverages language modeling, semantic search, and recommendation systems to measure and mitigate an analyst's exposure to concepts they find traumatic. Through a formative study of TIQA with 15 participants, we illuminate the complexities of enacting TIC in qualitative knowledge infrastructure, and potential roles for machine assistance in mitigating researchers' trauma. To assist scholars in translating the high-level principles of TIC into sociotechnical system design, we argue for: (a) a conceptual shift from safety as exposure reduction towards safety as enablement; and (b) renewed attention to evaluating the trauma-informedness of design processes, in tandem with the outcomes of designed objects on users' well-being.

==> 5_discussion-practical.tex <==
\subsection{Practical Recommendations for Developing Trauma-Informed Qualitative Coding Software}
\label{sec:dis-software-implications}
\enote{I'm actually not too sure what to do with this---right now it's just restating the low-level feedback. Thinking of striking it in favor of focusing the discussion on the higher-level points on design}
\nnote{I'm fine with removing this stuff. Or at least not having it first (can some of it be worked into Findings? Or perhaps mentioned as next steps for TIQA in limitations? i.e., I'm not sure reviewers would want there to be nothing in reaction to the feedback. But agree it should not start the discussion section since it's not the most interesting thing.) However, without this, the Discussion is pretty short, right? Would you add more? The CHI reviews had quite a bit of feedback about Discussion.}

In addition to theoretical extensions for the TIC literature, our work surfaced practical considerations for the research and development of tools for trauma-informed qualitative coding. In particular, we encourage further research into:

\subsubsection{Mechanisms for trauma-informed workload allocation under privacy constraints} \enote{how to deal with the quantification issue. are there crypto techniques that would work here?}

\subsubsection{Sustainable support for stakeholder-guided research on research-related harm}
Our study invited researchers with experience doing potentially traumatic research to collaborate on the design of tools to mitigate their traumatic exposure. \enote{some meta on doing this respectfully}

\enote{this is just the chaff summarizing the feedback}
As summarized in \tabref{tab:feature-feedback}, our formative study highlighted a range of design opportunities in how qualitative coding can become more trauma-informed.
Participants were initially quick to highlight the potential pitfalls of using ML in qualitative coding, in particular issues of bias and overreliance.
However, when presented with \artifactname as a tool using ML for semi-automated content warnings, participants viewed machine assistance as a ``\textit{value-add}'' (P06).
Having \artifactname provide measurements of prior and upcoming traumatic exposures could help researchers self-reflect on their own traumas and plan their own self-care practices, participants said---but they were mixed on whether counts of potentially traumatic phrases could provide the valid measurements they needed.
\artifactname's affordances for automatic nudges towards taking a break were seen as unhelpful: participants said they would immediately ignore or dismiss the nudges.
Instead, participants wanted to use \artifactname to scaffold collaborative practices in coding workflows, like borrowing models from peers, or using the self-reflection afforded by measurements of traumatic exposure to kickstart supportive conversations between fellow coders.
These measurements could also be used to allocate coding workloads to minimize individual coders' exposures, participants said, if and only if individual coders' privacy was also preserved.


==> 5_discussion-roles.tex <==
\subsection{\rev{Map complementary roles for humans and machines in trauma mitigation}}
\label{sec:dis-roles}
\rev{

The question of safety-as-enablement is an especially salient conceptual shift for projects involving mixed-initiative systems, like \artifactname. 

The literature on human-machine complementarity suggest carefully circumscribing human and machine roles in a mixed-initiative system, to maximize each side's contributions relative to their abilities and avoid mixing them. 
\citet{zerilli2019algorithmic}, for example, suggest humans should ``\textit{stick to what they do best}'' (e.g., communication, symbolic reasoning, conceptualization, empathy and intuition). \citet{zerilli2019algorithmic} also emphasize systems should remain dynamic to evolving capabilities on both sides: in other words, human users and machine components should be able to hand subtasks back to each other). 

Our formative study findings (\secref{sec:findings}) echo this separation of concerns. 
Participants alternated between envisioning desired roles for \artifactname (e.g., initiating collaborations between peers, serving as a surface for self-reflection) and cautioning against undesired roles (e.g., enforcing task efficiency, leaking private information between coders).
In both ML-assisted coding generally and the tracing of traumatic exposure specifically, participants wanted \artifactname to serve as a \textit{reflective surface} for their own analytic insights and psychosomatic reactions.



Future work might consider merging available principles and interaction guidelines for mixed-initiative systems (e.g., \citet{horvitz1999principles} and \citet{amershi2019guidelines}) with emerging guidance on trauma-informed computing (e.g., \citet{chen2022trauma} and \citet{scott2023trauma}).

}


==> 5_discussion-theoretical.tex <==
\input{figures/tab-safety-tradeoffs}

\subsubsection{Reframing from safety as exposure reduction towards safety as enablement}
\label{sec:dis-safety-collision}
% Existing literature advocates for a holistic and contextual approach to applying the six principles of TIC
The trauma literature understands \textit{safety} as both physical and psychological, encompassing both an internal sense of security and the absence of external harm \cite{chen2022trauma, scott2023trauma}.
In line with this definition, \artifactname's key affordances centered \textit{safety} by reducing users' traumatic exposure, via features like semi-automated content warnings personalized to their specific sensitivities, and nudges towards self-care after personalized exposure thresholds (\tabref{tab:safety-rationales}).
% several of our participants' suggested features---automatic content filters, allocating workloads to minimize traumatic exposure, or nudges towards self-care that actually lock an analyst out of their coding workflow---seem to reduce an analyst's traumatic exposure, thereby improving their \textit{safety}. 

Emphasizing safety in this way would seem vital to the core goal of the tool, to mitigate trauma, and how well it aligned with trauma-informed computing.
Yet, in analyzing how well \artifactname reflected TIC's six principles, we found these features created design rationales forcing tradeoffs between \textit{safety} and every other TIC principle. 
Semi-automatic content warnings or nudges towards self-care embody the reduction of traumatic exposure, but also seem to hamper users' agency, violating the principle of \textit{enablement}.
This core tension between safety and agency was also echoed across other principles.
Take, for example, the basic premise of machine assistance in content warnings.
ML-powered warnings were seen to create problems of \textit{trust}, because it is well known that ML can ``\textit{make mistakes and be horribly biased}'' (P14).
Participants also perceived that less experienced researchers might overrely on machine assurances and forgo the work of personalizing the tool, limiting their \textit{collaboration} in creating their technology experience.
Such overreliance could also encourage users to withdraw from the peer relationships that previously supported their self-care, violating \textit{peer support}.
Lastly, with respect to \textit{intersectionality}, it is possible an ML-powered content warning system may account for just one of a user's intersecting identities, and fail to warn them of content related to another facet of their experience.
% ---e.g., a tool may inadvertently show to a queer Asian woman content from Asian creators that is homophobic in nature.

To complicate matters, slight variations in how a feature is viewed can lead an analyst to conclude that safety has been favored or deprioritized relative to other principles.
Take, for instance, the previous example of collisions between \textit{safety} and \textit{enablement}.
Rather than understanding ML-assisted content warnings to reduce \textit{enablement} in favor of \textit{safety}, an analyst could conclude that since the user has some control over \artifactname's features (e.g., turning them off, reducing notification frequency), the tool actually prioritizes \textit{enablement} at \textit{safety's} behest. 
% \textit{enablement}: the ability to turn nudges on or off, or customize their own content filters via model training,  
% But increased user control necessitates some level of traumatic exposure that could harm \textit{safety}.
This malleability is not localized to the tradeoff between safety and enablement: for every TIC principle, we found possible design rationales favoring or deprioritizing safety across \artifactname's initial affordances (\tabref{tab:safety-rationales}).
A tool could support users' needs for improved \textit{trust} in ML-powered content warnings by introducing tools for explainability and transparency---but for users to do the work of understanding the model through these methods, they would need to expose themselves to some form of content that could also be traumatic, harming safety.
This same exposure problem hampers potential design decisions that emphasize \textit{collaboration} and \textit{intersectionality}: co-creation of technology experience, for example by providing the tool with enough annotated examples to accurately reflect one's situated sensitivities, inherently requires traumatic exposure that could harm safety.
Finally, to encourage \textit{peer support} and deemphasize user-to-machine overreliance, a tool could build in collaborative workflows that allocate datasets between coders---but doing so would require attention to privacy between teammates, to avoid unwanted exposure of an individual researcher's traumas to their colleagues.

These tradeoffs indicate a need to shift the conceptual frame of \textit{safety}, to accommodate its complicated interaction with other principles.
We consider that safety in technologies for trauma mitigation is perhaps best understood less as the shielding or removal of harmful experiences, and more as the provision of tools enabling users to manage safety for themselves: a conceptual shift we call \textbf{\textit{safety-as-enablement}}.
Conceptualizing safety in this way draws our focus towards using traumatic exposure measurements as surfaces for self-reflection and collaboration, as our participants were inspired to do, and helps alleviate the tensions between traumatic exposure and trauma-informedness we observe in \tabref{tab:safety-rationales}.
This widened aperture is also in concordance with the feminist approach to safety outlined in \citet{strohmayer2022safety}, which suggests embedding design friction into users' interactions with data-hungry platforms: specifically, the notion of a `\textit{trust pause}', during which users have a chance to critically reflect on whether to trust a system with their data.
A high-enablement interaction paradigm like this flouts typical design guidelines towards instantaneous reduction of burden via technology, but \citet{strohmayer2022safety} argue the short-term cost is to the longer-term benefit of maintaining users' trust in the system.

Importantly, safety defined as increased enablement may not be appropriate for all users: as prior work has described, in many situations, people may not want technologies to actually create extra work for them \cite{dombrowski2016social, tseng2020we}.
Still, as our work highlights, there may be unique benefits to encouraging enablement in technologies that scaffold potentially traumatic experiences: in the context of technology, enablement is fundamental, and opens opportunities for the other elements of trauma-informedness, namely peer support, collaboration, intersectionality.
We suggest that \textbf{safety-as-enablement} might ignite further design possibilities, both in qualitative coding software specifically and in trauma-informed design broadly, and encourage further interrogation of how TIC's principles might be adapted in this direction.



==> defs.tex <==
\renewcommand{\paragraph}[1]{\vspace*{6pt}\noindent\textbf{#1.}\;}

\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\apref}[1]{Appendix~\ref{#1}}
\newcommand{\fixme}[1]{\ifnum\authnote=1{\textcolor{red}{[FIXME: #1]}}\fi}
\newcommand{\better}[1]{\ifnum\authnote=1{\textcolor{violet}{[BetterWord: #1]}}\fi}
\newcommand{\todo}[1]{\ifnum\authnote=1{\textcolor{red}{[TODO: #1]}}\fi}

\newcommand{\new}[1]{\textcolor{blue}{#1}}

\newcounter{mynote}[section]
\newcommand{\notecolor}{blue}
\newcommand{\thenote}{\thesection.\arabic{mynote}}

\newcommand{\myemph}[1]{\vspace*{3pt}\emph{\textbf{#1}}\hspace*{3pt}}

\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}

\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{newitemize}{%
  \begin{list}{\mbox{}\hspace{5pt}$\bullet$\hfill}{\labelwidth=15pt%
      \labelsep=5pt \leftmargin=20pt \topsep=3pt%
      \setlength{\listparindent}{\saveparindent}%
      \setlength{\parsep}{\saveparskip}%
      \setlength{\itemsep}{3pt} }}{\end{list}}


\newenvironment{newenum}{%
  \begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=17pt%
      \labelsep=5pt \leftmargin=22pt \topsep=3pt%
      \setlength{\listparindent}{\saveparindent}%
      \setlength{\parsep}{\saveparskip}%
      \setlength{\itemsep}{2pt} }}{\end{list}}

%% ------------------------- Emily -----------------------

\newcommand{\enote}[1]{\ifnum\authnote=1\refstepcounter{mynote}{\textbf{\textcolor{blue}{$\ll$ET~\thenote: {\sf #1}$\gg$}}}\fi}

%% ------------------------- Nicki -----------------------

\newcommand{\nnote}[1]{\ifnum\authnote=1\refstepcounter{mynote}{\textbf{\textcolor{red}{$\ll$ND~\thenote: {\sf #1}$\gg$}}}\fi}

%% ------------------------- Tom -----------------------

\newcommand{\tnote}[1]{\ifnum\authnote=1\refstepcounter{mynote}{\textbf{\textcolor{orange}{$\ll$TR~\thenote: {\sf #1}$\gg$}}}\fi}

%% ------------------------ Revisions --------------------

\newcommand{\rev}[1]{\ifnum\revview=1{\color{blue}{#1}}\else{#1}\fi}

%% ------------------------ After Major Revisions --------------------

\newcommand{\revtwo}[1]{\ifnum\revtwoview=1{\color{blue}{#1}}\else{#1}\fi}

% This paper specific

\newcommand{\artifactname}{\textsc{TIQA}\xspace}



==> figure-descriptions.tex <==
Figure 1: Architectural diagram of how TIQA enables users to develop personalized models of their codes using the common underlying ML workflow. See Section 3.1 for a step-by-step walkthrough, and Table 2 for detail on each module.
Figure 2: Architectural diagram of how TIQA enables users to self-manage their traumatic exposure using the common underlying ML workflow. See Section 3.2 for a step-by-step walkthrough, and Table 2 for detail on each module.
Figure 3: Architectural diagram of how TIQA enables an analyst to view a data subject's current preferences for how their data is used in research. This feature also uses the common underlying ML workflow. See Section 3.3 for a step-by-step walkthrough.
Table 1: Mapping of design goals to the features of TIQA where they are realized; the principles of trauma-informed computing each feature enacts; and the figure where each feature is depicted in more detail.
Table 2: Modules of TIQA, their roles within the overall system design, and our approach to implementing them in the present tool.
Table 3: Participant demographics table.


==> figures/tab-participants.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\centering
\small
% \resizebox{\columnwidth}{!}
{%
\begin{tabular}{@{}lllllll@{}}
\toprule
\textbf{ID} & \textbf{Age} & \textbf{Gender} & \textbf{Fields} & \textbf{Preferred qual coding tools} & \textbf{Selected scenario} \\ \midrule
P01 & 26 & Woman & HCI, social computing & \begin{tabular}[c]{@{}l@{}}Excel and Notion; disliked Dovetail\end{tabular} & AOC's replies \\ \midrule
P02 & 24 & Woman & HCI, social computing & Ad hoc Shiny apps & AOC's replies \\ \midrule
P03 & 23 & Woman & Security and privacy & \begin{tabular}[c]{@{}l@{}}Notion; disliked Dedoose\end{tabular} & IPV case records \\ \midrule
P04 & 26 & Man & Security and privacy & \begin{tabular}[c]{@{}l@{}}Google Sheets; disliked NVivo\end{tabular} & IPV case records \\ \midrule
P05 & 30 & Woman & Social work, policy & \begin{tabular}[c]{@{}l@{}}Spreadsheets, Post-It notes,\\verbal debriefs; disliked NVivo\end{tabular} & IPV case records \\ \midrule
P06 & 28 & Woman & Security and privacy & \begin{tabular}[c]{@{}l@{}}Spreadsheets; disliked NVivo\\ \& MaxQDA (too expensive)\end{tabular} & AOC's replies \\ \midrule
P07 & 27 & Woman & Security and privacy & \begin{tabular}[c]{@{}l@{}}Dedoose; disliked NVivo\end{tabular} & IPV case records \\ \midrule
P08 & 36 & Non-binary & HCI, social computing & Google Sheets & AOC's replies \\ \midrule
P09 & 29 & Woman & \begin{tabular}[c]{@{}l@{}}NLP, computational social science\end{tabular} & \begin{tabular}[c]{@{}l@{}}Google Sheets, Airtable, MaxQDA\end{tabular} & IPV case records \\ \midrule
P10 & 27 & Woman & \begin{tabular}[c]{@{}l@{}}NLP, computational social science\end{tabular} & Prodigy, Excel & AOC's replies \\ \midrule
P11 & 38 & Woman & HCI, social computing & \begin{tabular}[c]{@{}l@{}}Word, Excel, Google Sheets;\\disliked QDAminer (needed \\more collaborative features)\end{tabular} & AOC's replies \\ \midrule
P12 & 30 & Woman & Security and privacy & \begin{tabular}[c]{@{}l@{}}Excel, Google Sheets;\\ disliked NVivo (needed more\\ collaborative features)\end{tabular} & AOC's replies \\ \midrule
P13 & 31 & Woman & HCI, social computing & \begin{tabular}[c]{@{}l@{}}Excel, Google Sheets\\Post-It notes; disliked NVivo\end{tabular} & AOC's replies \\ \midrule
P14 & 34 & Woman & \begin{tabular}[c]{@{}l@{}}NLP, computational social science\end{tabular} & Prodigy, Potato & AOC's replies \\ \midrule
P15 & 25 & Woman & Security and privacy & Excel & IPV case records \\ \bottomrule
\end{tabular}%
}
\caption{Relevant demographic and experiential characteristics of study participants.}
\label{tab:participants}
\end{table}

==> figures/tab-tic-design-goals.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\small
\centering
% \resizebox{\columnwidth}{!}
{%
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Design Goal} & \textbf{\artifactname Feature} & \textbf{TIC Principles} & \textbf{Description Key} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Enabling personalized\\ definitions of potentially\\ traumatic concepts\end{tabular} & \begin{tabular}[c]{@{}l@{}}User builds a model for concepts they personally \\ find traumatic by annotating examples.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Intersectionality,\\ Enablement\end{tabular} & A, B1 (Figure 1) \\ \cmidrule(l){2-4} 
 & \begin{tabular}[c]{@{}l@{}}User may opt to initialize their model from a \\ trusted peer's, to avoid the work of annotating \\ for traumatic concepts.\end{tabular} & Peer support & A (Figure 1) \\ \midrule
\begin{tabular}[c]{@{}l@{}}Supporting an analyst's \\ self-management of their \\ traumatic exposure\end{tabular} & \begin{tabular}[c]{@{}l@{}}Tool measures user's prior exposures to their \\ personally traumatic concepts.\end{tabular} & Safety & B2, B3 (Figure 1) \\ \cmidrule(l){2-4} 
 & \begin{tabular}[c]{@{}l@{}}Tool forecasts user's upcoming exposures, and \\ warns them how much potentially traumatic \\ content is to come.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Safety, \\ Enablement\end{tabular} & B2, B3 (Figure 1) \\ \cmidrule(l){2-4} 
 & \begin{tabular}[c]{@{}l@{}}Tool prompts user to log when they have a \\ reaction to their traumatic exposure, and \\ step away to take a break.\end{tabular} & Enablement & B4 (Figure 1) \\ \cmidrule(l){2-4} 
 & \begin{tabular}[c]{@{}l@{}}Tool uses the exposure measurements and \\ reaction logs in a personalized prediction for \\ when the user will next need a break, and nudges\\ them to engage in self-care then.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Safety, \\ Enablement,\\ Intersectionality\end{tabular} & B5 (Figure 1) \\ \midrule
% \begin{tabular}[c]{@{}l@{}}Respecting a data subject's \\ privacy preferences, \\ while still providing an\\ analyst with enough \\ context to do research\end{tabular} & \begin{tabular}[c]{@{}l@{}}For each document, a ``datasheet'' describes what \\ topics the data subject would NOT want their data \\ used to study.\end{tabular} & Collaboration & C (Figure 2) \\ \cmidrule(l){2-4} 
 % & \begin{tabular}[c]{@{}l@{}}Text segments reflecting forbidden topics are \\ grayed out. The analyst may view them for context \\ while pursuing different research questions, but \\ knows they may not be used otherwise.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Trust, \\ Collaboration\end{tabular} & C1, C2 (Figure 2) \\ \bottomrule
\end{tabular}%
}
\caption{Mapping of design goals to the features of \artifactname in which they are realized, the principles of trauma-informed computing each feature enacts, and the figure where each feature is depicted in more detail in the paper.}
\label{tab:tic-design}
\end{table}

==> privacy_design.tex <==
\subsection{Design Goal \#3: Respecting a data subject's preferences, while still enabling research} 
\label{sec:system-privacy}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/tiqa_C.drawio.pdf}
    \caption{Architectural diagram of how \artifactname enables an analyst to view a data subject's current privacy preferences, using the same underlying ML workflow (blue box) as in the features for personalized code modeling (\figref{fig:tiqa_A}) and traumatic exposure tracking (\figref{fig:tiqa_B}). See \secref{sec:system-privacy} for a step-by-step walkthrough.}
    \label{fig:tiqa_C}
\end{figure}

Mitigating the systems-induced trauma of qualitative research also requires attending to data subjects' preferences. 
Data subjects should be given agency over how their information is used and reused; however, when they release their information to a research repository, they have no way to know what it will be used to study in the future (\secref{sec:relwork-privacy}).
Existing approaches to enabling dynamic consent might include allowing data subjects to redact information that is categorically sensitive; however, this approach restricts analysts' ability to fully understand the context of the data, and reduces the creative freedom required of research.
The alternative, releasing unedited datasets with only personally identifiable information (PII) removed, helps protect data subjects' anonymity, but can still expose intimate details that they may not have wanted to release to the analyst, or which they did not want used within particular types of studies.
To redesign this process, we looked to the TIC principles of \textit{collaboration}, which holds that designers should create spaces for shared decision-making, and \textit{trust}, which holds that users (analysts in our context) should be given the opportunity to understand why a system works the way it does. 

\artifactname first surfaces a data subject's preferences to an analyst in the form of a datasheet, which depicts research topics for which the data subject would \textit{not} like to participate.
For example, an IPV survivor may wish to participate in general research on technology abuse, but not in specific research about family dynamics in IPV. 
Such preferences might be collected during informed consent processes or in other ways; we discuss this issue further in later sections.
\artifactname then models each preference as a code, and uses SemanticSearch to locate segments that match restricted concepts~(\textbf{C1}).
Matching segments are then grayed out on the document, to visually indicate that an analyst should exercise caution when reading that part of the document, with a note indicating which restricted concept they reflect (\textbf{C2}).
Thus, the tool enacts \textit{collaboration}, by creating a space where an analyst can understand and account for a data subject's preferences.
Further, to actualize \textit{trust}, \artifactname describes why each grayed-out section was selected: which topic the data subject would prefer that segment is not used to study.

==> privacy_findings.tex <==
\subsection{\artifactname can help balance researcher and subject interests, but requires accountability}
\label{sec:findings-privacy}
Participants were more receptive to the use of ML to help them respect data subjects' preferences than in general annotation tasks.
Many reported spending tremendous time and effort to protect their participants, utilizing 
practices like removing personally identifiable information, anonymizing quotes, obtaining informed consent, and securely storing sensitive datasets.

Participants appreciated the idea of enabling research on certain segments while flagging that other segments should not be used to study certain topics, based on the data subject's preferences.
This idea was particularly concordant for participants who chose the IPV case record dataset.
P12, who studies the privacy and security needs of vulnerable populations, said \artifactname's affordances would be particularly useful for similar datasets of deeply emotional interviews, for which a data subject might be embarrassed about an outburst, but still want to contribute to research.

\begin{quote}
    ``\textit{I love that you can have participants be like, `I do not want anybody to pay attention to the way that I'm emotionally responding to the situation, thanks.' And then, you can still use the rest of the information, without studying how they feel about XYZ.}'' (P12)
\end{quote}

Participants who chose the social media scenario were also interested in data subjects having more agency over the use of their information.
For many, broadcasting information on the Internet seemed like an irrevocable disclosure, and the challenge of realizing the \artifactname workflow lay upstream of the analyst's interface, in mechanisms for securing post-by-post preferences from users. As P06 said:

\begin{quote}
    ``\textit{[This feature] would require such a different landscape of how social media works. Like if every time a user posted something on Twitter or TikTok, they laid out what they're okay with their data being used for...it's not impossible, just not currently happening.}'' (P06)
\end{quote}

Assuming \artifactname \textit{could} obtain a data subject's preferences (a topic outside the scope of the present interface), participants were divided on how they should be surfaced to analysts.
Most agreed \textit{reducing} visibility into a flagged segment, by graying out segments of text (\figref{fig:tiqa_C}), was more palatable than \textit{eliminating} visibility, e.g., censoring or erasing blocks of text. 
Reduced visibility seemed to sufficiently signal to an analyst that that segment should be handled more delicately, while allowing them the context they needed to fully understand the data.
Some, however, were concerned any attempts to signal less-permissive parts of the data would in fact draw more attention to them. As P05 said, ``\textit{Does [a segment] being labeled forbidden actually sensationalize it?}''

Regardless of the visibility reduction technique, participants were concerned about how \artifactname could \textbf{validate} which sections should be de-emphasized.
Several said the ultimate decider should be the data subject, no matter how much this would constrain an analyst's creative freedom, because a data subject's agency in research mattered more. As P06 said, ``\textit{If [having less data] impacts the research, that sucks, but the whole point is that it impacts the research.}''
Others, however, felt that validation should fall under an analyst's purview, as part of a researcher's expertise. As P11 said: ``\textit{I'm the researcher. It's my decision whether this [segment] is actually [the prohibited concept] or not.}'' 

Importantly, several participants pointed out there were many cases where an analyst would \textit{want} to study data that a subject wanted to keep from scrutiny. 
For example, participants who study online political movements said revealing the beliefs of hate actors would be in line with the public interest, but might run afoul of the data subject's preferences.
The task, then, was for \artifactname to help an analyst decide when the public interest override might apply.

Towards resolving these issues, many participants suggested \artifactname could be accompanied by measures for \textbf{accountability}, surfacing to data subjects, collaborators, and broader research communities what an analyst did with a dataset.
Establishing transparency around the use of information in research would be a meaningful starting point for broader discussion of what norms and policies \artifactname should enact.
